New Interpretable Patterns and Discriminative Features from Brain Functional Network Connectivity Using Dictionary Learning

Independent component analysis (ICA) of multi-subject functional magnetic resonance imaging (fMRI) data has proven useful in providing a fully multivariate summary that can be used for multiple purposes. ICA can identify patterns that can discriminate between healthy controls (HC) and patients with various mental disorders such as schizophrenia (Sz). Temporal functional network connectivity (tFNC) obtained from ICA can effectively explain the interactions between brain networks. On the other hand, dictionary learning (DL) enables the discovery of hidden information in data using learnable basis signals through the use of sparsity. In this paper, we present a new method that leverages ICA and DL for the identification of directly interpretable patterns to discriminate between the HC and Sz groups. We use multi-subject resting-state fMRI data from $358$ subjects and form subject-specific tFNC feature vectors from ICA results. Then, we learn sparse representations of the tFNCs and introduce a new set of sparse features as well as new interpretable patterns from the learned atoms. Our experimental results show that the new representation not only leads to effective classification between HC and Sz groups using sparse features, but can also identify new interpretable patterns from the learned atoms that can help understand the complexities of mental diseases such as schizophrenia.

==> tmp.tex <==
\newpage




We are interested in the problem of sensor placement for signal estimation. 
We assume that the signal we measure $ s(t) $ is a scalar function of time. We have already placed $ K $ sensors measuring the signal with different gains 
$ \vect{a}_{K}= \left[a_1\, \cdots \, a_K\right]^{\T} $ 
and with spatially correlated noise. The sensors are placed at positions $\matr{X}_{K}=\left[\vect{x}_1\,\cdots \, \vect{x}_K \right] $ and the space where sensors are positioned is assumed to be $ D $-dimensional,  
$ \vect{x}_i\in \Rbb^{D} $. The vector of time measurements is
\begin{multline}
\vect{y}(\matr{X}_K,t)=\left[a_1\,\cdots\, a_K\right]^{\T}s(t)+[n(\vect{x}_1,t)\,\cdots\, n(\vect{x}_K,t)]^{\T}\\
=\vect{a}_{K}s(t)+\vect{n}_{K}(t)
\label{measurement}
\end{multline}
We assume that the noise is i.i.d. in time and second-order stationary in space and we want to choose $ N $ new sensor positions $\matr{X}_{N}=\left[x_1^{\star}\,\cdots \, x_N^{\star} \right]^{\T} $ such that signal estimation performance is enhanced.

\subsection{Source extraction by a linear estimator}
Without any further assumption on $ s(t) $, we can estimate it using all the measurements for any time $ t_i $ using the standard linear estimator. Consider $ \vect{f}_{K+N} $ to be the linear estimator parameter corresponded to the estimation parameter at a specific positions $\matr{X}_{K+N}=\left[\matr{X}_{K} \matr{X}_{N} \right] $. Therefore, the estimation of the source becomes as follows:
\begin{equation}
\hat{s}(t_i)=\vect{f}_{K+N}^T ~ \vect{y}(\matr{X}_{K+N},t_i)
\label{linear_estimator}.
\end{equation}
By replacing \eqref{measurement} in the above equation, we have the following:
\begin{multline}
\hat{s}(t_i)=\vect{f}_{K+N}^T ~ (\vect{a}_{K+N}s(t_i)+\vect{n}_{K+N}(t_i)) = \\
\vect{f}_{K+N}^T \vect{a}_{K+N}s(t_i) + \vect{f}_{K+N}^T\vect{n}_{K+N}(t_i)
\label{linear_estimator_for_SNR}.
\end{multline}

To find the estimation parameter $ \vect{f}_{K+N} $, we calculate the signal to noise ratio (SNR) of the above estimation which is desired to be as maximum as possible. Then the estimation parameter can be extracted by taking the derivative of the resulted SNR. The SNR of \eqref{linear_estimator_for_SNR} is as follows:

\begin{equation}
\text{SNR} = \frac{\mean\left[({\vect{f}_{K+N}^T \vect{a}_{K+N}s(t_i)})^2\right]}{\mean\left[({\vect{f}_{K+N}^T\vect{n}_{K+N}(t_i)})^2\right]} = 
\frac{(\vect{f}_{K+N}^T \vect{a}_{K+N})^2 \sigma_s^2}{\vect{f}_{K+N}^T \matr{C}^n_{K+N} \vect{f}_{K+N}}
\label{SNR}
\end{equation}
where $ \sigma_s = \mean\left[ \vect{s}(t) \vect{s}(t)^T \right]$ is the variance of the source with respect to the time and $ \matr{C}_{K+N}^{n} = \mean\left[ \vect{n}_{K+N}(t) \vect{n}_{K+N}^T(t) \right]$ is the spatial covariance of the noise at the set of sensor positions $ \matr{X}_{K+N} $. Note that $ \matr{C}_{K+N}^{n} $ can be partitioned in $ 4 $ matrix blocks
\begin{equation}
\matr{C}_{K+N}^{n}=\left[\begin{array}{cc}
\matr{C}_{KK}^{n}& \matr{C}_{KN}^{n}\\
(\matr{C}_{KN}^{n})^{\T}& \matr{C}_{NN}^{n}\end{array}\right]
\end{equation}
corresponding to the covariance between noise samples for the initial set of sensors $ \matr{C}_{KK}^{n} $, to the sensors to be added $ \matr{C}_{NN}^{n} $ and to the covariance $ \matr{C}_{KN}^{n} $ between both. Vector $ \vect{a}_{K+N}=\left[\vect{a}_{k}^{\T}\, \vect{a}_{N}^{\T}\right]^{\T}  $ is also the extended vector of gains. Now, by taking the derivative of \eqref{SNR} and set it equal to zero, it is straightforward to show that the the estimation parameter is proportional to $ ( \matr{C}_{K+N}^{n})^{-1} \vect{a}_{K+N} $. More precisely, $\vect{f}_{K+N} = \lambda (  \matr{C}_{K+N}^{n})^{-1} \vect{a}_{K+N} $ where $ \lambda = \frac{\vect{f}_{K+N}^T  \matr{C}_{K+N}^{n}  \vect{f}_{K+N} }{\vect{f}_{K+N}^T \vect{a}_{K+N}} $. Since the coefficient factor $ \lambda $ doesn't have any effect in the value of SNR and also it just behaves as a scale in the estimation of the source, we can consider $ \lambda $ to be equal to one, and consequently the estimation parameter becomes:
\begin{equation}
\vect{f}_{K+N} = (\matr{C}_{K+N}^{n})^{-1} \vect{a}_{K+N},
\label{f}
\end{equation}
By replacing \eqref{f} in \eqref{linear_estimator}, the estimated source using linear estimator with respect to maximizing the corresponding SNR becomes as follows:
\begin{equation}
\hat{s}(t_i)= \vect{a}_{K+N}^T (\matr{C}_{K+N}^{n})^{-1} ~ \vect{y}(\matr{X}_{K+N},t_i)
\label{linear_estimator1}.
\end{equation}
Also, from \eqref{SNR}, the SNR becomes as follows:
\begin{equation}
\text{SNR}=  \sigma_s^2 \vect{a}_{K+N}^T (\matr{C}_{K+N}^{n})^{-1}\vect{a}_{K+N}.
\label{SNR1}.
\end{equation}

If the gain vector $ \vect{a}$ was perfectly known, then we could evaluate the SNR at all possible positions according to the above equation. Consequently, after finding the optimal position for allocating the new sensor, the best estimation of the source could be achieved using \eqref{linear_estimator1}. However, in reality, we do not have the exact values for $ \vect{a}_{K+N} $. To deal with this obstacle, it is necessary to assume a model for the gain vector. Kriging model is one of the classical methods to achieve this goal. in the next subsection, the Kriging model is described to model the gain vector $ \vect{a} $.

\subsection{Kriging model}
Clearly, the sensor gains may also have spatial dependence and we need to integrate this through a model. One way for doing so is by assuming a stochastic model for the underlying continuous gain function $ a(\vect{x}) $. In what follows we suppose that the gain function $ a(\vect{x}) $ is a stationary Gaussian process around a trend function:
\begin{equation}
a(\vect{x})\sim \mathcal{GP}\left[ m(\vect{x}),\,\matr{C}^{a}(\vect{x},\vect{x}')\right] 
\label{gp}
\end{equation}
where $ m(\vect{x}) $ is the mean-vector modeling the trend. For example, it can be a linearly parametrized function
\begin{equation}
m(\vect{x})=\sum\limits_{i=1}^{p} \beta_i f_i(\vect{x})
\label{mean_function}
\end{equation}
where $ \beta_i $ are parameters and $ f_i(\vect{x}) $ are fixed functions. Note that the functions can be non-linear. The kernel function $ \matr{C}^{a}(\vect{x},\vect{x}') $ specifies the covariance matrix of the Gaussian process at any two points $ \vect{x}$ and $\vect{x}'$. Different types of kernel are reported in the literature \cite{stein2012interpolation,rasmussen2006gaussian}. Depending on the behavior of the underlying gain function, we use a different kernel. For example, if we want to model a rather smooth gain function with infinitely differentiable sample-paths, we can use the following squared exponential kernel:
\begin{equation}
\matr{C}^{a}(\vect{x},\vect{x}')=\sigma_a^2\exp\left[-\dfrac{1}{2}r(\vect{x,\vect{x}'})\right]
\label{squared_exponential}
\end{equation}
where $ r(\vect{x,\vect{x}'})=(\vect{x}-\vect{x}')^T\Diag{\vect{\rho}_{a}}^{-1} (\vect{x}-\vect{x}') $ and $ \vect{\rho}_{a}=\left[\rho_{a}^{(1)} \, \cdots \, \rho_{a}^{(D)}\right]^T $ is a vector with correlation length-scales for the different spatial axes. Parameter $ \sigma_a $ is the standard deviation of the process and thus controls the amplitude of its fluctuations around $ m(\vect{x}) $.

This type of model is known as Kriging \cite{krige1951statistical}. It was original used in mining applications and it is now used in many different fields.

Since the noise is also spatial dependent, we can also assume that it follows a Gaussian process with its own parameters.
\begin{equation}
n(\vect{x})\sim \mathcal{GP}\left[ 0,\,\matr{C}^{n}(\vect{x},\vect{x}')\right] 
\label{gp_noise}
\end{equation}

The use of a stochastic model serves in general for two purposes:

\begin{itemize} 
	\item \emph{Interpolation:} to be able to interpolate $ a(\vect{x}) $ from observed $ \vect{a}_{K} $ at any set of candidate points. Since $ a(\vect{x}) $ is a stochastic process, this can be done in a Bayesian way. If we want to give the best estimate $ \vect{a}_{N}=\vect{a}(\matr{X}_{N})=\left[\hat{a}(\vect{x}_{1}^{\star})\,\cdots\,\hat{a}(\vect{x}_{N}^{\star})\right]^T  $ in MSE sense at the positions $ \matr{X}_{N} $, then this is given by the posterior (conditional) mean:
	\begin{equation}
	\hat{\vect{a}}(\matr{X}_{N})=\mean\left[\vect{a}(\matr{X}_{N})|\vect{a}_{K} \right] 
	\label{predict_general}
	\end{equation}
	\item \emph{Uncertainty quantification:} to quantify the level of uncertainty on the estimated gain function at a set of points $ \matr{X}_{N} $. This is naturally given by the posterior covariance:
	\begin{multline}
	\matr{C}^{\vect{a}_{N}|\vect{a}_{K}}=\\
	\mean\left[\left( \vect{a}(\matr{X}_{N})-\hat{\vect{a}}(\matr{X}_{N})\right)\left( \vect{a}(\matr{X}_{N})-\hat{\vect{a}}(\matr{X}_{N})\right)^T|\vect{a}_{K} \right] 
	\label{covariance_general}
	\end{multline}
\end{itemize}

Moreover, the Gaussian assumption simplifies greatly the evaluation of these two quantities, since they are given in closed-form expressions. Using the partition of the posterior covariance, the estimate of the gains is
\begin{equation}
\hat{\vect{a}}(\matr{X}_{N})=\vect{m}(\matr{X}_{N})+\matr{C}_{KN}^{a}\left(\matr{C}_{KK}^{a}\right)^{-1}(\vect{a}_{K}-\vect{m}(\matr{X}_{K}))
\label{predict_kriging}
\end{equation}
where $ \vect{m}(\vect{X}_{N})=[m(\vect{x}_{1}^{\star})\,\cdots\,m(\vect{x}_{N}^{\star})]^T $ and $ \vect{m}(\vect{X}_{K})=[m(\vect{x}_{1})\,\cdots\,m(\vect{x}_{K})]^T $. While its posterior covariance is given by
\begin{equation}
\matr{C}^{\vect{a}_{N}|\vect{a}_{K}}=\matr{C}_{NN}^{a}-\matr{C}_{NK}^{a}\left(\matr{C}_{KK}^{a}\right)^{-1}\left(\matr{C}_{NK}^{a}\right)^T
\label{covariance_kriging}
\end{equation}
Observe that we have assumed that the parameter vector in the trend $ \vect{\beta} $ is known. If it is unknown, then we can estimate it with the data and the expressions (\ref{predict_kriging}) and (\ref{covariance_kriging}) need to be slightly modified, see \cite{ohagan1978curve} for details.

It is noticeable that (\ref{predict_kriging}) and (\ref{covariance_kriging}) are valid whenever we perfectly know the value of gain $ \vect{a}_K $ at the initial pints. However, if we do not have the exact values for $ \vect{a}_K $, the best estimation for $ \vect{a}_{K+N} $ is the mean $ \vect{m}_{K+N} $ which we know from the Gaussian assumption on gain vector $ \vect{a} $. In the numerical section both situations will be examined and compared to each other.

\subsection{Criterion function for sensor placement}
In the classical kriging methods, the common criterion is defined in such a way that minimizes the variance over the mean of the model presented in \eqref{gp}. Also, other state of the arts use other criteria such as mutual information (MI). For example the proposed method in \cite{Krause2008NOSP} attempts to select the new positions in such a way that maximizes the increase in mutual information. However, all these criteria are focused on minimizing the uncertainty caused by the selected model for gain $ \vect{a} $. However, in the purpose of the source estimation, the main goal is not to perfectly model the gain vector $ \vect{a} $, but the attempt is to have the best estimation of the source. Therefore, these classical methods are not able to cover the effect of the environmental noise $ \vect{n}(t) $. In this paper, we take this fact into account. So, the idea is that instead of targeting the variance of estimated $ \vect{a} $, we maximize the SNR of the estimated source $ s(t) $.

Given $ K $ previously placed sensors with the knowledge of the exact values for gains $ \vect{a}_K $ at these initial positions, if we want to place $ N $ new sensors then the vector $ \vect{a}_{K+N} $ is partly deterministic and partly random. The SNR then becomes a random variable, which is dependent on the choice of $ \matr{X}_{N} $. So, we should choose a meaningful statistic of it to maximize. The straightforward option\footnote{Other options based on quantiles of this random variable may exist but they require a precise determination of its underlying distribution.} is to maximize its expectation conditioned on the already known spatial gains:
\begin{multline}
J(\matr{X}_{N})=\mean\left[ \vect{a}_{K+N}^T(\matr{C}_{K+N}^{n})^{-1}\vect{a}_{K+N}|\vect{a}_{K}\right]\\
= tr \lk (\matr{C}_{K+N}^{n})^{-1} \mean\left[ \vect{a}_{K+N} \vect{a}_{K+N}^T|\vect{a}_{K}\right]  \rk.
\label{J_criterion}
\end{multline}
The above equation is valid whenever we perfectly know the value of $ \vect{a}_K $. However, as already mentioned, we do not have such precise information. Therefore, according to our knowledge, the only information we have is the position of the initial sensors, as well as the mean of the Gaussian assumption on the gain vector $\vect{a}$. Therefore, the best estimation that we can have for gains would be $ \hat{\vect{a}}_{K+N} = \vect{m}_{K+N} $. Consequently, we rewrite \eqref{J_criterion} as follows:
\begin{multline}
J(\matr{X}_{N})= tr \lk (\matr{C}_{K+N}^{n})^{-1} \mean\left[ \vect{a}_{K+N} \vect{a}_{K+N}^T|\matr{X}_{K} , \matr{X}_{N}  \right]  \rk.
\label{J_criterion_main}
\end{multline}
Doing some mathematical calculations, it is straightforward to shown that:
\begin{multline}
\mean\left[ \vect{a}_{K+N} \vect{a}_{K+N}^T|\matr{X}_{K} , \matr{X}_{N} \right] = \matr{C}^a_{K+N} + \vect{m}_{K+N} \vect{m}_{K+N}^T,
\label{C+mm'}
\end{multline}
where $\matr{C}^a_{K+N}$ and $ \vect{m}_{K+N}$ are respectively the corresponding covariances and means from \eqref{gp}. Therefore, the new position which maximizes the defined target function \eqref{J_criterion_main} is the near optimal position to achieve the maximum SNR. 
